Outer Billiards on Kites

Outer billiards is a simple dynamical system based on a convex planar shape. The Moser-Neumann question, first posed by B.H. Neumann around 1960, asks if there exists a planar shape for which outer billiards has an unbounded orbit. The first half of this monograph proves that outer billiards has an unbounded orbit defined relative to any irrational kite. The second half of the monograph gives a very sharp description of the set of unbounded orbits, both in terms of the dynamics and the Hausdorff dimension. The analysis in both halves reveals a close connection between outer billiards on kites and the modular group, as well as connections to self-similar tilings, polytope exchange maps, Diophantine approximation, and odometers.

==> 5fun2.tex <==


\section{Proof of Theorem \ref{discrete}}
\label{fundamental2}

\subsection{The Pivot Theorem}
\label{statepivot}

Given an odd rational parameter $A=p/q$,
let $V$ be the vector from Equation
\ref{boxvectors}.  Let $\Z V$ denote
the group of integer multiples of $V=(q,-p)$.
In Part VI we prove the following result.

\begin{theorem}[Pivot]
Every low vertex of $\Gamma$ is equivalent mod
$\Z V$ to a vertex of $P\Gamma$. That is,
$P\Gamma$ contains one period's worth of low
vertices on $\Gamma$.
\end{theorem}

The Pivot Theorem makes a dramatic
statement. Another way to state the Pivot Theorem is that
there are no low vertices on the complementary
arc $\gamma-P\Gamma$. Here $\gamma$ is the arc
just to the right of $P\Gamma$ such that
$P\Gamma \cup \gamma$ is one full period of
$\Gamma$.  A glance at Figure 23.1 will make
this clear.  
We will prove the Pivot Theorem in Part VI.  We will
also prove the following easy estimate.

\begin{lemma}
\label{pivotbound}
$$
\label{pivotbind}
-\frac{q}{2}<\pi_1(E^-)<\pi_1(E^+)<\frac{q}{2}.
$$
\end{lemma}

See \S \ref{formulapivot}.
Here $E^+$ and $E^-$ are the pivot points, defined in
\S \ref{pivots}.

\subsection{The Inheritance of Low Vertices}

Let $A_1 \leftarrow A_2$ be two odd rationals.
  Let $\widetilde V_1=V_1$ if
$A_1<A_2$ and $\widetilde V_1=-V_1$ if $A_1>A_2$.
Let 
\begin{equation}
d_1={\rm floor\/}(q_2/2q_1).
\end{equation}

Let $v_1$ be a vertex on the pivot arc 
$P\Gamma_1$. Define
\begin{equation}
v_2=v_1+k \widetilde V_1; \hskip 30 pt
k \in \{0,...,d_1\}.
\end{equation}
Notice that these were precisely the vertices that
we considered in \S \ref{cantorformula}.   Now
we want to take a close look at these vertices.
Here is the main result of this section.

\begin{lemma}
\label{low}
$v_1$ is low with respect to $A_1$ iff $v_2$ is low
with respect to $A_2$.
\end{lemma}

\startproof
There are two cases to consider, depending on whether
$A_1<A_2$ or $A_2<A_1$.  We will consider the former
case.  The latter case has essentially the same
treatment.  In our case, we have $\widetilde V_1=V_1$.
Let $E_j^{\pm}$ be the pivot points for $\Gamma_j$.
Say that a vertex is {\it high\/} if it is not low.

We will first suppose that $v_1$ is low with respect
to $A_1$ and that $v_2$ is high with respect
to $A_2$.  This will lead to a contradiction.
We write $v_j=(m_j,n_j)$.  Let $M_j$ be
the fundamental map from Equation \ref{funm}.
Since $v_1$ is
low and $v_2$ is high, we have
$$
2A_1m_1+2n_1+\frac{1}{q_1}=M_1(v_1) \leq 2-\frac{1}{q_1};$$
$$
2A_2m_2+2n_2+\frac{1}{q_2}=M_2(v_2) \geq 2+\frac{1}{q_2}.
$$
Rearranging terms, 
\begin{equation}
\label{case11}
2\bigg(\frac{p_2}{q_2}m_2+n_2\bigg)-2\bigg(\frac{p_1}{q_1}m_1+n_1\bigg) \geq \frac{2}{q_1}.
\end{equation}
Plugging in the relations $m_2=m_1+kq_1$ and $n_2=n_1-kp_1$ and simplifying, we get
\begin{equation}
\label{case22}
\frac{(m_1+kq_1)(p_2q_1-p_1q_2)}{q_1q_2} \geq \frac{1}{q_1}.
\end{equation}
Since $A_1 \leftarrow A_2$ and $A_1<A_2$, we have
\begin{equation}
\label{case33}
p_2q_1-p_1q_2=2.
\end{equation}
Hence
\begin{equation}
\label{precon}
m_1+kq_1 \geq \frac{q_2}{2}.
\end{equation}
Combining Equation \ref{pivotplus} and Equation
\ref{precon}, we get
$$
E_1^+(A_2)=E_1^+(A_1)+d_1q_1 \geq^* m_1+kq_1>\frac{q_2}{2}>^*E_1^+(A_2).$$
This is a contradiction.
the first starred inequality comes from the Pivot 
Theorem and the fact that $k \leq d_1$.  The second
starred inequality comes from the Corollary \ref{pivotbound}.

Now we will suppose that $v_1$ is high with respect to
$A_1$ and $v_2$ is low with respect to $A_2$.  This
will also lead to a contradiction.  Let $M_1$ denote
the first coordinate of the fundamental map relative
to the parameter $A_1$, adjusted so that $M_1(0,0)=1/q_1$. That is
\begin{equation}
M_1(m,n)=2A_1m+2n+\frac{1}{q_1}.
\end{equation}
Since $v_1$ is high, we have the following
dichotomy.
\begin{equation}
M_1(v) \geq 2+\frac{1}{q_1}; \hskip 30 pt
M_1(v)>2+\frac{1}{q_1} \hskip 12 pt
\Longrightarrow \hskip 12 pt
M_1(v) \geq 2+\frac{3}{q_1}.
\end{equation}
We will consider these two cases in turn.
\newline
\newline
{\bf Case 1:\/}
If $M_1(v_1)=2+1/q_1$, then 
$$M_1(m_1,n_1-1)=\frac{1}{q_1}=M_1(0,0).$$
But than $(m_1,n_1-1)=jV_1$ for some integer $j$.
But then $|m_1| \geq q_1$. Since
$v_1 \in P\Gamma_1$, this contradicts 
Corollary \ref{pivotbound}.
Hence $$v_1=(0,1); \hskip 30pt v_2=kV_1+(0,1).$$
If $v_2$ is low then
$$0=2k(A_1 q_1-p_1)<2k(A_2 q_1-p_1)=M_2(v_2)-M_2(0,1) \leq 0.$$
This is a contradiction.  The first inequality comes from
$A_1<A_2$.
\newline
\newline
{\bf Case 2:\/}
If $M_1(v_1) \geq 2+3/q$, then the same reasoning as
in Equations \ref{case11}, \ref{case22}, and \ref{case33} (but with
signs reversed) leads to 
\begin{equation}
m_1+kq_1<-3q_2.
\end{equation}
But then
$$
\frac{-q_2}{2}<\frac{-q_1}{2}<^*m_1 \leq m_1+kq_1<-3q_2
$$
The starred inequality comes from Corollary \ref{pivotbound}.
Again we have a contradiction, this time by a wide margin.
\endproof

\subsection{The End of the Proof}

 Let $\Lambda_n$ denote the
set of low vertices of $P\Gamma_n$.
By the Pivot Theorem, every low vertex on $P\Gamma_n$ is
equivalent to a point of $\Lambda_n$ modulo $\Z V_n$.

\begin{lemma}
\label{inductlow}
For any $n \geq 0$, we have
$$\Lambda_{n+1}=\bigcup_{k=0}^{d_n}(\Lambda_n+k \widetilde V_n).$$
\end{lemma}

\startproof
Induction.
For $n=0$ we have $E_1^-=(-d_0,d_0)$ and
$E_1^+=(0,0)$.  In this case, the right
hand side of our equation precisely describes
the set of points on 
the line segment joining the pivot points.
The case $n=0$ therefore follows directly
from the Pivot Theorem.

Let $\Lambda_{n+1}'$ denote the right hand side of
our main equation. Since
$\Gamma_n$ is invariant under translation by
$V_n$, every vertex of
$\Lambda_{n+1}'$ is low with respect to
$A_n$. Hence, by Lemma \ref{low}, every
vertex of $\Lambda_{n+1}'$ is low with
respect to $A_{n+1}$. 
 Combining this
fact with Equation \ref{copycorr}, we
see that 
$\Lambda_{n+1}' \subset \Lambda_{n+1}$.

By Lemma \ref{low} again, every $v \in \Lambda_{n+1}$
is also low with respect to $A_n$.  Hence
\begin{equation}
v=v'+k \widetilde V_n; \hskip 30 pt k \in \Z.
\end{equation}
for some $v' \in \Lambda_n$.  If
$k \not \in \{0,...,d_n\}$ then
$v$ either lies to the left of the left
pivot point of $\Gamma_{n+1}$ or to
the right of the right pivot point
of $\Gamma_{n+1}$.  Hence
$k \in \{0,...,d_n\}$.  This proves
that $\Lambda_{n+1} \subset \Lambda'_{n+1}$.
Combining the two facts completes our induction
step.
\endproof

We proved Lemma \ref{inductlow} with respect to the inferior
sequence.  However, notice that if $d_n=1$ then
$\Lambda_{n+1}=\Lambda_n$.  Thus, we get precisely the
same result for consecutive terms in the superior sequence.
We have shown that $v \in \Gamma_n$ is low if and only 
if $v \in \Lambda_n$ mod $\Z V$.  But then
\begin{equation}
O_2(1/q_n,-1) \cap I=M(\Lambda_n); \hskip 30 pt
I=[0,2] \times \{-1\}.
\end{equation}
Here $M$ is the fundamental map. 
Recognizing $\Lambda_n$ as the set from Equation \ref{total},
we get precisely the equality in Theorem \ref{discrete}.
There is one last detail.  One might worry that $M$ maps
some points of $\Lambda_n$ to points on $[0,2] \times \{1\}$,
but all points in $\Lambda_n$ have even parity. Hence,
this does not happen.

This completes the proof of Theorem \ref{discrete}.


\subsection{Theorem \ref{discrete} in the Even Case}
\label{extra}

Here we discuss Theorem \ref{discrete} in the even case.
For each even rational $A_1 \in (0,1)$ there is a unique
odd rational $A_2$ such that (in the language of
Equation \ref{induct0}) $A_1=(A_2)_{\pm}$ and
$q_2<2q_1$.  In Lemma \ref{welldefined} we will
show that $\Gamma_1$ (a closed polygon) contains a copy of
$P\Gamma_2$, and all low vertices of
$\Gamma_1$ lie on this arc.  
From this fact, we see that

\begin{equation}
O(1/q_1,-1)=M_1(\Sigma_1),
\end{equation}
just as in the odd case.  Here $M_1$ is the fundamental
map defined relative to the parameter $A_1$ and
$\Sigma_1$ is the set of low vertices on $P\Gamma_1$.

Note that $\Sigma_1=\Sigma_2$, where $\Sigma_2$ is the
set of low vertices on $P\Gamma_2$.  The only difference
between the two sets $M_1(\Sigma_1)$ and
$M_2(\Sigma_2)$ is the difference in the maps $M_1$
and $M_2$.  Now we explain the precise form of 
Theorem \ref{discrete} that this structure entails.

Switching notation, let
$A$ be an even rational.  One of the two rationals
$A_{\pm}$ from Equation \ref{induct0} is odd, and
we call this rational $A'$.  
We can find the initial part of a superior sequence
$\{A_k\}$ such that $A'=A_{n-1}$.  We set
$A=A_n$ even though $A$ does not belong to this sequence.
Referring to Theorem \ref{discrete}, we define $\Pi_n$
exactly in the odd case, but for one detail.  In
case $2q'>q$, we simply ignore the $n$th factor of
$\Pi_n$. That is, we treat $q'$ as an inferior term.
With these changes, Theorem \ref{discrete} goes through
word for word.

Here we give an example. Let $A_1=12/31$.  Then
$A_2=19/49$, exactly is in the introduction.  We have
$n=3$ and our sequence is
$$\frac{p_0}{q_0}=\frac{1}{1}, \frac{1}{3}, \frac{5}{13}, \frac{12}{31}=\frac{p_3}{q_3}.$$
All terms are superior, so this is also the superior sequence.
$n=3$ in our example, and the renormalization sequence is $1,2,1$.
The $\mu$ sequence is $19,5,1$.   The first coordinates of the
 $12$ points of 
$O_2(1/49) \cap I$ are given by 
$$\bigcup_{k_0=0}^1\  \bigcup_{k_1=0}^2\  \bigcup_{k_2=0}^1 \frac{2(19k_0+5k_1+1k_2)+1}{31}.$$
Writing these numbers in a suggestive way, the union above works out to
$$\frac{1}{31} \times \big(1\hskip 8pt 3\hskip 20 pt    11\hskip 8pt 13\hskip 20pt   21\hskip 8pt 23 \hskip 60 pt   
39\hskip 8pt 41\hskip 20 pt    49\hskip 8pt 51\hskip 20 pt    59\hskip 8pt 61\big).$$

\newpage




==> 6arc.tex <==


\section{Proof of the Short Arc Lemma}


\newpage


